Detecting Face Synthesis Using a Concealed Fusion Model

Face image synthesis is gaining more attention in computer security due to concerns about its potential negative impacts, including those related to fake biometrics. Hence, building models that can detect the synthesized face images is an important challenge to tackle. In this paper, we propose a fusion-based strategy to detect face image synthesis while providing resiliency to several attacks. The proposed strategy uses a late fusion of the outputs computed by several undisclosed models by relying on random polynomial coefficients and exponents to conceal a new feature space. Unlike existing concealing solutions, our strategy requires no quantization, which helps to preserve the feature space. Our experiments reveal that our strategy achieves state-of-the-art performance while providing protection against poisoning, perturbation, backdoor, and reverse model attacks.

==> DATA/FIGS/FIG_Artifacts.tex <==
\begin{figure}
\vspace{-10pt}
\includegraphics[width=\textwidth]{./DATA/FIGS/Artifacts.pdf}
\vspace{-10pt}
\caption{ \footnotesize{  Artifacts in synthetic face images (left to right): a large scar below the eye, a scar below the nose, a dented forehead, and uneven ears.  }  }
\vspace{-10pt}
\label{fig:appx}
\end{figure}



==> DATA/TABS/CNN.tex <==
\begin{table}
\centering
\vspace{-30pt}
\caption{\small{ Architecture of the proposed \acrshort{MLP} detector. } }
\label{table:mlp}
\resizebox{1\linewidth}{!}{
\begin{tabular}{llllll}
\toprule
Layer Type & Number of Filters & Feature Map Size & Kernel Size & Stride & Activation \\
\midrule
Input &  & $256 ^{2} \times 3$ &  &  &\\
Center-Crop &  & $224 ^{2} \times 3$ &  &  & \\
\midrule
Convolution Layer 1\textsuperscript{st} & $16$ & $224 ^{2} \times 16$ & $5 \times 5 $ & $1 \times 1$ & ReLu \\
\midrule
Convolution Layer 2\textsuperscript{nd} & $24$ & $220 ^{2} \times 24$ & $5 \times 5 $ & $1 \times 1$ & ReLu \\
\midrule
Convolution Layer 3\textsuperscript{th} & $32$ & $216 ^{2} \times 32$ & $5 \times 5 $ & $1 \times 1$ & ReLu \\
\midrule
Batch Normalization &&&&& \\
\midrule
Fully Connected Layer 1\textsuperscript{st} &  & $ 212 ^{2} \times 32 \rightarrow 120$ &  & & \\
%ReLu activation &&&& \\
\midrule
Fully Connected Layer 2\textsuperscript{nd} &  & $120 \rightarrow 84$ &  &  &\\
\midrule
Fully Connected Layer 3\textsuperscript{th} &  & $84 \rightarrow 2$ &  &  &\\
\bottomrule

\end{tabular}
}
\end{table} 

